When Good Components Go Bad: Formally Secure Compilation Despite Dynamic Compromise

We propose a new formal criterion for evaluating secure compilation schemes for unsafe languages, expressing end-to-end security guarantees for software components that may become compromised after encountering undefined behavior---for example, by accessing an array out of bounds. Our criterion is the first to model dynamic compromise in a system of mutually distrustful components with clearly specified privileges. It articulates how each component should be protected from all the others---in particular, from components that have encountered undefined behavior and become compromised. Each component receives secure compilation guarantees---in particular, its internal invariants are protected from compromised components---up to the point when this component itself becomes compromised, after which we assume an attacker can take complete control and use this component's privileges to attack other components. More precisely, a secure compilation chain must ensure that a dynamically compromised component cannot break the safety properties of the system at the target level any more than an arbitrary attacker-controlled component (with the same interface and privileges, but without undefined behaviors) already could at the source level. To illustrate the model, we construct a secure compilation chain for a small unsafe language with buffers, procedures, and components, targeting a simple abstract machine with built-in compartmentalization. We give a machine-checked proof in Coq that this compiler satisfies our secure compilation criterion. Finally, we show that the protection guarantees offered by the compartmentalized abstract machine can be achieved at the machine-code level using either software fault isolation or a tag-based reference monitor.

==> texdirectives.tex <==
\camerafalse\draftfalse\anonfalse

